Algebraic complete axiomatisation of ZX-calculus with a normal form via elementary matrix operations

In this paper we give a complete axiomatisation of qubit ZX-calculus via elementary transformations which are basic operations in linear algebra. This formalism has two main advantages. First, all the operations of the phases are algebraic ones without trigonometry functions involved, thus paved the way for generalising complete axiomatisation of qubit ZX-calculus to qudit ZX-calculus and ZX-calculus over commutative semirings. Second, we characterise elementary transformations in terms of ZX diagrams, so a lot of linear algebra stuff can be done purely diagrammatically.

==> mypackages.tex <==
\usepackage{amsmath, amsthm,amsfonts,amssymb,mathtools,mathdots}

\usepackage{tikz, stmaryrd,tabularx,enumitem}
\usetikzlibrary{shapes}

% theorem styles
%\newtheorem{thm}{Theorem}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem{lem}[thm]{Lemma}
%\theoremstyle{definition}
%\newtheorem{dfn}[thm]{Definition}
%\newtheorem{axgrp}[thm]{Axioms}
%\theoremstyle{remark}
%\newtheorem{remark}[thm]{Remark}
%\newtheorem{exm}[thm]{Example}
% end theorem styles

% tikz diagrams specification
\usetikzlibrary{arrows, decorations.markings, shapes.geometric, decorations.pathmorphing, decorations.pathreplacing, intersections, patterns,calc, backgrounds}

\pgfdeclarelayer{bg}
\pgfdeclarelayer{mid}
\pgfdeclarelayer{fg}
\pgfsetlayers{bg,mid,fg,main}

\tikzset{
	follow/.style={->, >=stealth, very thick, shorten <=3pt, shorten >=3pt, color=black},%magenta!80},
	edge/.style={line width=.8pt, color=black},
	edgedot/.style={densely dotted, line width=.8pt, color=black},
	edgethdot/.style={densely dotted, line width=.8pt, color=gray},
	edgeth/.style={line width=.8pt, color=gray!60},
	mirror/.style={line width=1.6pt, color=magenta!80},
	dot/.style={circle, draw=black, line width=.8pt, fill=white, inner sep=1.7pt},
	dotth/.style={circle, draw=gray!60, fill=gray!60, inner sep=1.25pt},
	dotwh/.style={circle, draw=gray!60, line width=.8pt, fill=white, inner sep=1.8pt},
	dotwhite/.style={circle, draw=gray, line width=.8pt, fill=white, inner sep=1.8pt},
	dotdark/.style={circle, draw, fill=black, inner sep=1.25pt},
	dotgrey/.style={circle, draw=black, line width=.8pt, fill=gray!60, inner sep=1.6pt},
	coverc/.style={circle, draw=gray, line width=.8pt, inner sep=3pt},
	coverch/.style={circle, draw=gray!30, line width=.8pt, inner sep=3pt},
	%% My definition
	none/.style={circle, draw=none},
	dotred/.style={circle, draw, fill=red, inner sep=1.5pt},
	dotredh/.style={circle, draw, fill=red!60, inner sep=1.5pt},
	dotgreen/.style={circle, draw, fill=green, inner sep=1.5pt},
	dotgreenh/.style={circle, draw, fill=green!60, inner sep=1.5pt},
	boxwhite/.style={rectangle, draw, fill=white, inner sep=3pt},
	boxyellow/.style={rectangle, draw, fill=yellow, inner sep=3pt},
	boxgreen/.style={rectangle, draw, fill=green, inner sep=3pt},
	boxred/.style={rectangle, draw, fill=red, inner sep=3pt},
	uptriyellow/.style={regular polygon,regular polygon sides=3, draw, fill=yellow, inner sep=1.5pt},
	downtriyellow/.style={regular polygon,regular polygon sides=3, draw, fill=yellow, inner sep=1.5pt,rotate=180},
	lefttriyellow/.style={regular polygon,regular polygon sides=3, draw, fill=yellow, inner sep=1.5pt,rotate=90},
	righttriyellow/.style={regular polygon,regular polygon sides=3, draw, fill=yellow, inner sep=1.5pt,rotate=-90},
	%%%%%
	dotthl/.style={circle, draw=gray!60, fill=gray!60, inner sep=0.8pt},
	dotwhl/.style={circle, draw=gray!60, line width=.8pt, fill=white, inner sep=0.8pt},
	dotwhitel/.style={circle, draw=gray, line width=.8pt, fill=white, inner sep=0.8pt},
	dotredl/.style={circle, draw, fill=red, inner sep=0.8pt},
	dotredhl/.style={circle, draw, fill=red!60, inner sep=0.8pt},
	dotgreenl/.style={circle, draw, fill=green, inner sep=0.8pt},
	dotgreenhl/.style={circle, draw, fill=green!60, inner sep=0.8pt},
	boxwhitel/.style={rectangle, draw, fill=white, inner sep=2pt},
	boxyellowl/.style={rectangle, draw, fill=yellow, inner sep=2pt},
	boxgreenl/.style={rectangle, draw, fill=green, inner sep=2pt},
	boxredl/.style={rectangle, draw, fill=red, inner sep=2pt},
	every node/.style={scale=.8},
	every picture/.style={scale=.8},
}
% end tikz diagrams specification

% Specific categories
%\newcommand\cat[1]{\mathbf{#1}}
%\newcommand\graded{\cat{Hilb}^{\mathbb{Z}_2}}

% Other
\newcommand\blankline{\vspace{6pt}}
%\newcommand\comment[1]{\textcolor{magenta}{$^{[\text{#1}]}$}}

%\newcommand\dagg[1]{#1^\dagger}

%\newcommand\braket[2]{\langle\, #1 \,|\, #2 \,\rangle}
%\newcommand\bra[1]{\langle\, #1\,|}
%\newcommand\ket[1]{|\, #1 \, \rangle}
%\newcommand\ketbra[2]{\ket{#1} \! \bra{#2}}
%\newcommand\upto{\underset{\,\diamond}{=}}
%\renewcommand*{\arraystretch}{1.2}

%\linespread{1.05}

